The spatially resolved PAH characteristics in the Whirlpool Galaxy (M51a)

We present a detailed study on the spatially resolved polycyclic aromatic hydrocarbon (PAH) emission properties in the (circum)nuclear region (NR) and extranuclear regions (ENRs) of M51a using Spitzer-IRS observations. Correlations among PAH intensity ratios are examined with respect to each other, local physical parameters, galactocentric distance ($R_{g}$), and very small grain (VSG) emission. Additional comparison is performed with the mid-infrared emission features in the H$_{\mathrm{II}}$ regions of M33 and M83. The NR exhibits the strongest correlation among the PAH intensity ratios, whereas ENRs are showing increased scatter attributed to ISM emission. Overall, the radiation field hardness has a higher impact on PAH emission than metallicity, with the latter regulating PAH variance as a function of $R_{g}$. Specifically, the variance of PAH emission with respect to the different physical parameters suggests a higher rate of small/medium PAH processing compared to large PAHs and a higher ratio of small-to-large PAHs formed with increasing galactocentric distance. We find similarities between the 7.7 $\mu$m carriers in M51a's NR and M83's H$_{\mathrm{II}}$ regions, the 8.6 $\mu$m carriers in M51a's NR and M33 H$_{\mathrm{II}}$ regions, and both types of carriers between M51a's ENRs, M33's, and M83's H$_{\mathrm{II}}$ regions. We have identified a positive correlation between PAH/VSG and the PAH intensity ratios. We conclude that the relative abundance of PAHs and VSG is not solely driven by the hardness of the radiation field.

==> RevisedAbstract.tex <==
We present a detailed study on the spatially resolved polycyclic aromatic hydrocarbon (PAH) emission properties in the (circum)nuclear region (NR) and extranuclear regions (ENRs) of M51a using <i>Spitzer</i>-IRS observations. Correlations among PAH intensity ratios are examined with respect to each other, local physical parameters, galactocentric distance (R<sub>g</sub>), and very small grain (VSG) emission. Additional comparison is performed with the mid-infrared emission features in the H<sub> II</sub> regions of M33 and M83. The NR exhibits the strongest correlation among the PAH intensity ratios, whereas ENRs are showing increased scatter attributed to ISM emission. Overall, the radiation field hardness has a higher impact on PAH emission than metallicity, with the latter regulating PAH variance as a function of R<sub>g</sub>. Specifically, the variance of PAH emission with respect to the different physical parameters suggests a higher rate of small/medium PAH processing compared to large PAHs and a higher ratio of small-to-large PAHs formed with increasing galactocentric distance. We find similarities between the 7.7 μm carriers in M51a's NR and M83's H<sub> II</sub> regions, the 8.6 μm carriers in M51a's NR and M33 H<sub> II</sub> regions, and both types of carriers between M51a's ENRs, M33's, and M83's H<sub> II</sub> regions. We have identified a positive correlation between PAH/VSG and the PAH intensity ratios. We conclude that the relative abundance of PAHs and VSG is not solely driven by the hardness of the radiation field.

